Grid Peeling of Parabolas

Grid peeling is the process of repeatedly removing the convex hull vertices of the grid-points that lie inside a given convex curve. It has been conjectured that, for a more and more refined grid, grid peeling converges to a continuous process, the affine curve-shortening flow, which deforms the curve based on the curvature. We prove this conjecture for one class of curves, parabolas with a vertical axis, and we determine the value of the constant factor in the formula that relates the two processes.

==> general-curves.tex <==


Try to get inspiration from the techniques from 
 ..Calder and Smart~\cite{cs-lschp-20},

... translate it into simpler terms for
the special case of two dimensions and uniform density $f\equiv 1$.
 
 ..``what we call semiconvex peeling.'' (p.2090)
 In Section 2, we study a related peeling process called semiconvex peeling.

1.3. Game interpretation

convex hull game, 

3.2. Simple test functions

We build our test functions by distorting $\phi$ = parabola.

``test functions'' for approximating ACSF.
the idea is not only to apply an affine transformation to
the geometry, but also to apply a /convex/concave function to time.


3.3. Piecewise approximation

I think the core thing to prove is an analog of
Lemma 3.9. In our setting

Look at sec.4 (10 pages) for ideas 

4. Convex peeling

4.1. Comparison lemmas


4.3. Scaling limit
We now prove our main theorem by combining the piecewise approximations from
Section 3 with the above barrier lemmas. 
 The essential idea is that piecewise subsolutions and supersolutions form global barriers for the convex peeling.
 = approximation from above and below. / from inside and outside

\hrule

\paragraph{Next step. Arbitrary curves}
Take the outer envelope of a couple of local inner approximations.
On the other side, the inner envelope of a couple of local outer approximations.
...

Maybe we can try the circle, for a start.
I think the idea is to approximate the ACSF from inside and outside.

Let us try the circle
$$
(x-1)^2+(y-1)^2 = 2$$
at one of its points: the origin.

The osculating parabola (through the origin) is of the form
%$$y = a(x-1)^2 -$$is
$$y = ax^2 +bx$$
$$y' = 2ax +b$$
Match the slope of the circle
$$y'(0) = b=-1$$
$$y = ax^2 -x$$
We insist that the point $x_0\to 0$,
$y_0(x_0) = ax_0^2 -x_0$
lies on the circle
$$
(ax_0^2 -x_0 -1)^2 + (x_0 -1)^2 = 2
$$
$$
a^2x_0^4 -2ax_0^3 + x_0^2 -2ax_0^2 +2x_0 +1+ x_0^2 -2x_0 +1= 2
$$
\begin{equation}
a^2x_0^4 -2ax_0^3 + 2x_0^2 -2ax_0^2  = 0
\end{equation}
Ignoring the (double) root $x_0=0$:
\begin{equation}
a^2x_0^2 -2ax_0 + 2 -2a  = 0
\end{equation}
[Equivalently,
\begin{equation}\label{eq-x0}
(ax_0-1)^2 + 1 -2a  = 0 ]
\end{equation}
We want to solve this for $a$, for $x_0\to 0$
$$
a^2x_0^2 -2a(1 + x_0) + 2 = 0
$$
$\to a=1$.
Thus, the osculating parabola is:
$$y = x^2 -x = (x-\tfrac12)^2 -\tfrac14$$

One of $a=1\pm\eps$ should locally give an inner approximation,
the other an outer approximation.

Take  $a=1+\eps$ ($\eps$ can be negative)
and solve \eqref{eq-x0} for $x$ ($=x_0$).
General solution:
$$
x = \big(1 \pm \sqrt{2a-1}\big) / a
$$
We are interested in the solution near $x=0$:
$$
x = \big(1 - \sqrt{2a-1}\big) / a
$$
(The other intersection point is $x=2, y=2$, the opposite point on the circle.
These two opposite points are the points where the osculating parabola exits the circle.)

Substitute
$a=1+\eps$:  %($\eps$ could be negative)
$$
x = \big(1 - \sqrt{1+ 2\eps}\big) / ( 1+\eps)
= -\eps + 3/2 \cdot \eps^2 +O(\eps^3)
$$
according to sage.
% sage: taylor((1-sqrt(1+2*x))/(1+x),x,0,4)                                      % 21/8*x^4 - 2*x^3 + 3/2*x^2 - x

For $a=1+\eps>1$ (larger curvature), the parabola crosses the circle near $x\approx -\eps<0$,
touches it \emph{from inside} at the origin, and crosses it again near $(2,2)$.
INNER local approximation. makes sense. See Figure~\ref{fig:osculating}.

For $a=1-\eps<1$ (smaller curvature), the parabola
touches \emph{from outside} at the origin,  crosses the circle near $x\approx\eps>0$, and crosses again near $(2,2)$.
OUTER local approximation.

\begin{figure}
    \centering
    \includegraphics{osculating.pdf}
    \caption{
    osculating parabola at the origin,
    local outer approximation 
    near the origin ($a=1-\eps$),
    and
    local inner approximation ($a=1+\eps$).
    In the two right pictures, the parabola touches the circle
    in the origin but does not cross it.
    The pictures are drawn
    for rather large $\eps$, but still one can barely
    distinguish the curves between the two intersection points}
    \label{fig:osculating}
\end{figure}

Each approximation is valid for an interval of size $\approx \eps$.
[What is the approximation error, in an interval of length $\delta$ around
the osculating point? $O(\delta^3+\eps\delta^2)$?]

Q: Can INNER approximations be combined/stitched together to form a *convex* approximation?
Or we don't need to care about convexity
using the notion of
subpeeling sequence from Section~\ref{sec:subpeeling}?

\subsection{Parabolas with slanted axes}

REMARK: For the OUTER approximation of the circle, we might resort to unimodular transformations, which can turn the parabola axis in any (rational) direction that we like, and which leave the validity of Theorem~\ref{main-parabola} unchanged.
(The vertex of the parabola is the point
of maximum curvature.)
But this works only for the circle, and only for the other approximation.

We could also apply a unimodal transformation to ``turn'' parabolas.
E.g., $(\begin{smallmatrix}
    1&1\\0&1
\end{smallmatrix})$
leads to a $45^\circ$ axis.
In this way, on could deal WITH THE CIRCLE, from OUTSIDE only,
using true (global) approximation from outside for a dense family of directions.
\subsection{Local approximations}

Outer approximations seem easy to be stitched together.
Several outer (local) approximations
with parabolas similar to
Figure~\ref{fig:osculating} middle, but touching the circle at different (close together)
points,
can be easily combined to form a piecewise parabolic outer (in this case: lower)
approximation.

Such ``lower'' (and ``upper'') outside approximations
would be used for the part of the curve (circle) where the slope is between $-1$ and $1$.
In the other two quartercircles one would use approximations
from ``left'' and ''right''.

Increasing the ``density'' (and therefore precision)
of these approximations does not cost anything; they can be as
dense as we want.

It seems obvious that one can combine the local motions from several adjacent parabolas,
using the notion of
superpeeling from Section~\ref{sec:subpeeling}.

TECHNICAL PROBLEM: each local approximation is not valid globally.
E.G. the parabola in the middle of Figure~\ref{fig:osculating} reenters the
circle (near the lowest point of the circle, in this case).

How to prove that this does not matter? How much do we lose from 
Theorem~\ref{main-parabola}, if we consider, for example, the curve
\begin{equation}\label{parabola-with-straight}
    y = \begin{cases}
    x^2 & \text{for $x\ge 0$}\\
    0 & \text{for $x\le 0$}
    \end{cases}
\end{equation}
over the interval $1\le x\le 2$?
Depending on $n$, how many steps can we go before the
difference to the parabola $y=x^2$ is felt at all at $x=1$?

As a conservative subpeeling approximation, one could even hold
the $y=0$ for $x\le 0$ fixed.

See Figure \ref{fig:boundary-effects}.

From parabolic pieces whose ends are straightened, like
in \eqref{parabola-with-straight}, one could approximate the circle
correctly, and the argument would work easily with superpeeling.

I think, also the ACSF for \eqref{parabola-with-straight} at $x=1$ proceeds EXACTLY like for $y=x^2$, for a certain positive time.
The influence of the change in $x<0$ creeps only gradually to the right with time.
(1. This is in contrast to the first quadrant case in Section 
\ref{sec:hyperbolas}, where the curve IMMEDIATELY lifts off the two axes, all the way to infinitly.
2. An argument might be based on the affine erosion model mentioned in the introduction,
sec 1.1.)

\begin{figure}
    \centering
    \noindent\hskip-1,52cm\includegraphics[scale=0.8]{boundary-effects.pdf}
    \caption{An example of ``boundary effects''. Both on the left
    edge and on the right edge, these are different
    effects than what is required to study here.
    They result from incorrect treatment
    of the interval boundaries in the simulation program. Still they illustrate
    the point: The effect of the boundaries works its way more and more inward
    with time.}
    \label{fig:boundary-effects}
\end{figure}

\subsection{Superpeeling and Subpeeling}
\label{sec:subpeeling}

\input{superpeeling}

\hrule


==> horizontal-period.tex <==

% APPENDIX:
%\section{The Horizontal Period for a Parabola}
% (HAS NOW BEEN MOVED TO THE MAIN PART)

\begingroup
\setcounter{proposition}{\propPeriod}
\addtocounter{proposition}{-1}

\begin{proposition}[restated]
 Consider the parabola
 \begin{equation} \label{parabola}
    y=\frac{a_N}{a_D}x^2 +
  \frac{b_N}{b_D}x + c     
 \end{equation}
with reduced fractions $\frac{a_N}{a_D}$ and $\frac{b_N}{b_D}$.


  The horizontal period $H$ is either equal to
  $\bar H := \lcm(a_D,b_D)$ or to
  $\bar H/2$. In particular
  \begin{enumerate}
  \item
[(i)]
    If $a_D\equiv 0 \pmod 4$, then $H = \lcm(a_D/2,b_D)$.
  \item [(ii)]
 If $a_D\equiv 2 \pmod 4$
and $b_D\equiv 2 \pmod 4$,
    then $H = \lcm(a_D/2,b_D/2)$.
  \item [(iii)]
In all other cases,  $H = \lcm(a_D,b_D)$.
  \end{enumerate}
  
  
\end{proposition}

\endgroup

  \begin{proof}
  Since vertical lines should remain vertical
  and vertical distances should remain unchanged,
  the affine transformation that we are looking for has
  the form
  \begin{equation} \label{transformation} 
        \begin{aligned}
      x & \mapsto x+z\\
      y & \mapsto y + ux + w
  \end{aligned}
  \end{equation}
  for suitable parameters $z,u,w$.
    Substituting the right-hand sides of \eqref{transformation} for $x$ and $y$ should leave \eqref{parabola} unchanged.
 This leads to the following equations for $u$ and $v$:
    \begin{align}
      \label{eq:u}
      u &= 2\tfrac{a_N}{a_D}z
%      \in \mathbb Z
\\
%and
%    \begin{equation}
      \label{eq:w}
      w &= \tfrac{a_N}{a_D}z^2 + \tfrac{b_N}{b_D}z 
%      \in \mathbb Z.
    \end{align} %    \end{equation}   
The additional requirement is that
integer grid points should be mapped to
integer grid points. This boils down to requiring that
 $z,u,w$ are integral.

Thus, the horizontal period $H$ that we are looking for
is the smallest positive integer $z$ for which the two quantities $u$
    and $w$ defined above
    are integers.

    It is easy to see that $z = \bar H = \lcm(a_D,b_D)$ will make both
 \eqref{eq:u} and
     \eqref{eq:w} integral. We have to check whether a smaller value
     also does the job.
We start with an easy observation:
    
 Observation A:
    If $z$ or the integer $u$ is even, then
    $w$ is an integer
 iff  $z$ is a multiple of $b_D$.

 Proof.
 We can rewrite \eqref{eq:w} in terms of $u$:
    \begin{equation}
      \label{eq:w2}
      w = \tfrac{uz}{2} + \tfrac{b_N}{b_D}z 
  %    \in \mathbb Z.
    \end{equation}
 If $uz$ is even, then
  the first term $\tfrac{uz}{2}$ in  \eqref{eq:w2} is an integer.
Therefore, for $w$ to be an integer, the second term
must also be an integer, which is the case iff $b_D$ divides $z$.

We will make a case distinction based on the parity of $a_D$:
    
Case 1: $a_D$ is even: Then $u$ is an integer iff $z$ is a multiple of
$a_D/2$.

Case 1.1: $a_D$ is a multiple of 4: Then $u$ is even, and
Observation A implies that
$w$ is an integer iff $b_D$ divides $z$.
Part~(i) follows.


Case 1.2:
$a_D\equiv 2 \pmod 4$.
Then $a_N$ must be odd,
because $\tfrac{a_N}{a_D}$ is reduced. Moreover,
 $u$ is an integer iff $z$ is a multiple of
the odd number $a_D/2$.

Now we distinguish two subcases, depending on the (unknown) value $z$.

Case 1.2.1: $z$ is odd. In this case,
$u=\frac{a_Nz}{a_D/2}$ is also odd, and
the first term $\tfrac{uz}{2}$ in  \eqref{eq:w2} is a half-integer
(a non-integer multiple of $1/2$).
For $w$ to be an integer, the second term
$\tfrac{b_Nz}{b_D}$
must also be a half-integer. This is only possible if the factor 2 is
contained in the denominator $b_D$. In this case, $b_N$ must be odd,
because $\tfrac{b_N}{b_D}$ is reduced. If $b_D$ is divisible by 4,
then the numerator $b_Nz$, which is odd, cannot cancel this factor,
and $\tfrac{b_Nz}{b_D}$ cannot be a half-integer.
Hence the only possibility is that
$b_D\equiv 2 \pmod 4$, i.e.,
Part~(ii) of the Proposition.
Then
$\tfrac{b_Nz}{b_D}$ is a half-integer iff
$\tfrac{b_Nz}{b_D/2}$ is an integer, which holds iff
$z$ is a multiple of
$b_D/2$.
This establishes that
the claimed value $\lcm(a_D/2,b_D/2)$, which is odd,
is the smallest viable value of $z$ in this case.

Case 1.2.2: $z$ is even. (This is an additional possibility for
Part~(ii), and the only remaining possibility as a subcase of Case 1.2 when
the conditions of
Part~(ii) don't hold.)

Since $z$ is even, it %Then $z$
must be a multiple of $\lcm(2,a_D/2)= a_D$.
Observation A implies that
$w$ is an integer iff $z$ is also a multiple of $b_D$.
Thus $z$ must be a multiple of $\bar H=\lcm(a_D,b_D)$.
This establishes that the value $\bar H/2$ for Case 1.2.1 is indeed the smallest
possible value when this case is possible,
i.e., in Part~(ii) of the Proposition.
When
Case 1.2.1 does not apply, this is in accordance with Part~(iii).

Case 2: $a_D$ is odd: Then $u$ is an integer iff $z$ is a multiple of
$a_D$, and $u$ will be even.
As above, Observation A implies that
$w$ is an integer iff $z$ is also a multiple of $b_D$.
The smallest possible value $z$ is
$\bar H=\lcm(a_D,b_D)$, and
this is in accordance with Part~(iii).    
  \end{proof}

    

==> proof-of-asymptotic.tex <==
%\section{Proof of Lemma~\ref{lem-Ht-asymptotic} about the asymptotic growth of \texorpdfstring{$H_t$}{H\_t}}
%\label{app-proof}

TO BE EVENTUALLY THROWN OUT, AFTER THE MATERIAL
HAS BEEN INTEGRATED IN THE MAIN TEXT.

% \begin{proof}[Proof of \eqref{expr-asymp-precise}]

%We denote by $\mathbb P=\{\,(i,j)\in \mathbb Z\times \mathbb Z \mid
%\gcd(i,j)=1\,\}$ the set of \emph{primitive vectors}.

Following \cite[p.~61]{sandor99},
% In a first step,
we reduce the computation of $H_t$ to
the estimation of the quantity~$R(u)$, which is defined as follows
for any real parameter $u$: %, cf. 
\begin{align}
 R(u) &:=
        \label{def-R}
    \sum_{\substack{ 1\le y\le x\le u\\(x,y)\in \mathbb P}}
  x\\&
  = \nonumber
    \sum_{\substack{ 1\le x\le u}}\,
    \sum_{\substack{ 1\le y\le x\\(x,y)\in \mathbb P}}
  x
  =
  \sum_{x=1}^{\lfloor u\rfloor}x\phi(x)
%  \\  
%&=    \sum_{x=1}^{\lfloor u\rfloor}\substack{(x,y)\in \mathbb P\\ 1\le y\le x\le u}}
%    x\\  
\end{align}
By regrouping and reformulating sums, we get:
\begin{align}
  H_t %&= %\#\{\,(x,y)\in \mathbb P \mid 0<x\le y\le t}
         \nonumber
  &=
    \sum_{\substack{  0<y\le x\le t\\(x,y)\in \mathbb P}}
  \left\lfloor \frac
  tx \right\rfloor x \\
  \nonumber
  &=
    \sum_{\substack{0<y\le x\le t\\(x,y)\in \mathbb P}} \,
  \sum_{\substack{k\ge 1\\ xk\le t}} x%\\  &
                                             =
    \sum_{{k\ge 1}} % \sum_{\substack{x\ge 1\\xk\le t}}
 \,   \sum_{\substack{ 0<y\le x\le t\\xk\le t\\(x,y)\in \mathbb P}}
  x%\\  &
          =
    \sum_{\substack{k\ge 1\\\ }}\,
    \sum_{\substack{ 0<y\le x\le t/k\\(x,y)\in \mathbb P}}
    x\\
  &=
    \sum_{k\ge 1} R(\tfrac tk) \label{H-to-R}
\end{align}
%(The same relation between $H_t$ and $R$ is used in the proof in
%\cite[p.~61]{sandor99}.)
For $R(u)$, we will use the following asymptotic estimate:
\begin{lemma}\label{lemma-R}
  \begin{equation}\label{R-asymp}
    R(u) =
     \sum_{1\le x \le u} x\phi(x)
     =
     \frac {2u^3}{\pi^2}
%     \frac {u^3}{3
     +O(u^2\log u)
\end{equation}
for $u\to\infty$.
\end{lemma}
Sándor and Kramer \cite[p.~61, \thetag{20}]{sandor99} derived this
asymptotic expression (without the error bound) as an easy consequence
of a general statement of Radoux~\cite{radoux77} about the sum
$\sum_{x=1}^u f(\tfrac xu)\phi(x)$ being asymptotically equal to
${6u^2}/{\pi^2}\int_{z=0}^1zf(z)\,dz$ for an arbitrary function $f$,
provided that $zf(z)$ is continuous.  (The deeper reason behind this
statement is that the fraction of primitive vectors among the integer
vectors in \emph{any} sufficiently large ``well-behaved'' region is
$1/{\zeta(2)}$, see also
Bárány and
Rote
\cite[Theorem~2]{br-scdpg-06} or
Har-Peled and Lidický
\cite[Lemma 2.2]{Har-Peled-Lidicky} for some explicit lower bounds.
%
Examples of well-behaved regions for which this statement holds
are convex regions with a limit on the ratio between incircle and
circumcircle, or dilates of a fixed convex region.)  We include an
elementary proof of Lemma~\ref{lemma-R} below, immediately after
using it to finish the estimation of $H_t$.

Substitution of
\eqref{R-asymp}
in \eqref{H-to-R} gives our claimed asymptotic formula for $H_t$:
\begin{align*}
  H_t & = \sum_{k\ge 1} R\bigl(\tfrac tk\bigr) %\\    &
        = \sum_{k\ge 1} \frac 2{\pi^2}\frac{t^3}{k^3}
+ \sum_{k\ge 1} O\bigl(\tfrac{t^2}{k^2}\log \tfrac tk \bigr)
 % \\&
  = \frac {2t^3\zeta(3)}{\pi^2} + O(t^2\log t)
%\qedhere
\end{align*} 
%\end{proof}

\endinput
 \begin{proof}[Proof of Lemma~\ref{lemma-R}]
   We use the notation $T(u)$ for the sum
\eqref{def-R}
   without the condition that
     $(x,y)$ should be primitive:
\begin{align}
 T(u) &:=
        \sum_{1\le y\le x\le u}  x
        \label{def-T}
 \\  
      &=    \sum_{x=1}^{\lfloor u\rfloor}x^2
      % \\&
  =
       \frac{ \lfloor u\rfloor^3}3 +\frac{\lfloor u\rfloor^2}2 +
  \frac{\lfloor u\rfloor}6
  \nonumber
  \\  &
                           = \frac {u^3}3 + O(u^2)
                           \label{T-approx}
\end{align}
 We claim that the $O(u^2)$ error term can be explicitly bounded by
\begin{equation}
  \label{bound-E}
  \bigl\lvert T(u)-\tfrac{u^3}3\bigr| \le
  E(u) :=
  \begin{cases}
%    \frac{u^2}2+\frac u6 \le
  \frac{u^3}3  & \text{for $0<u<1$} \\
    \frac{2u^2}3  & \text{for $u\ge 1$} \\
  \end{cases}
\end{equation}
The bound
for the first case, $u< 1$, is trivial because $T(u)=0$ in this case.
The bound
for the second case, $u\ge 1$,
can be checked by an easy computation:
\begin{align*}
T(u)&= \textstyle 
\frac{\lfloor u\rfloor^3}3+ \frac{\lfloor u\rfloor^2}2+\frac {\lfloor
      u\rfloor}6
      \le
      \frac{u^3}3+ \frac{u^2}2+\frac u6
      \le
      \frac{u^3}3+ \frac{u^2}2+\frac {u^2}6
  \\
T(u)&= \textstyle 
\frac{\lfloor u\rfloor^3}3+ \frac{\lfloor u\rfloor^2}2+\frac {\lfloor u\rfloor}6 \ge
\frac{(u-1)^3}3+ \frac{(u-1)^2}2+\frac {u-1}6
=\frac{u^3}3- \frac{u^2}2+\frac {u}6
      \ge
      \frac{u^3}3- \frac{u^2}2-\frac {u^2}6.
\end{align*}
%
and therefore,
%$-(\frac{u^2}2-\frac u6)\le T(u)-\frac{u^3}3\le \frac{u^2}2+\frac u6$.
%Hence,
$|T(u)-\frac{u^3}3|\le 
%\frac{u^2}2+\frac u6 \le
    \frac{2u^2}3$.



The following %We give an independent and more elementary
proof
of~Lemma~\ref{lemma-R}
follows the derivation of the similar formula
\begin{equation}
  \nonumber % \label{eq:sum-phi}
    \sum_{\substack{ 1\le y\le x\le u\\(x,y)\in \mathbb P}}
  1
=    \sum_{x=1}^{\lfloor u\rfloor}\phi(x)
=\frac {u^2}{2\zeta(2)}+O(u\log u) \sim
\frac {3u^2}{\pi^2}
\end{equation}
in \cite[Theorem~330]{HW}, a result that goes back to Mertens in 1874.
% Journal für Math. 77 (1874)m 289--338.
% (Landau, Handbuch der Lehre von der Verteilung der Primzahlen, 2
% Bände, Teubner, Leipzig 1909, 578--9)
% error term has been reduced to smaller power of log (Walfisz 1963)
%

%, except that we do not use Euler's $\phi$-function explicitly.

%the Möbius function $\mu$ explicitly but use
%inclusion-exclusion directly.

Comparing
\eqref{def-R}
with the sum~\eqref{def-T}, for which we have an explicit formula, we
want to exclude
the vectors $(x,y)$ that are not primitive, i.e., where both $x$ and $y$ are
 multiples of one of the primes $2,3,5,7,11,\ldots$.
By the inclusion-exclusion formula,
we have to
subtract the contribution of those vectors that are divisible by
 $2$, by 3, by 5, etc., add the vectors that are divisible by \emph{two}
 primes, subtract the vectors that are divisible by three primes, etc.
The contribution of the vectors that are divisible by $n$ is $nT(\frac
un)$, as these vectors are all integer vectors from the smaller region
$0< y\le x\le u/n$, scaled by~$n$.
We obtain:
 \begin{align*}
   R(u) &= T(u) - \bigl(2T(\tfrac u2) + 3T(\tfrac u3) + 5T(\tfrac u5) + \cdots
          \bigr)\\
   &\qquad
   + 
     \bigl(2\cdot 3\cdot  T(\tfrac u{2\cdot 3}) +
     2\cdot 5\cdot  T(\tfrac u{2\cdot 5}) +
     \cdots \bigr)
\\   &\qquad
   -
   \bigl(2\cdot 3 \cdot 5\cdot  T(\tfrac u{2\cdot 3\cdot 5}) + \cdots \bigr) + \cdots
   \\
   &= \sum_{n=1}^\infty \mu(n) n T(\tfrac un),
 \end{align*}
 In the last line, we have expressed the alternating sum
 % of terms of the form $nT(\frac un)$
 in terms of the Möbius function
 \begin{displaymath}
   \mu(n) =
   \begin{cases}
     +1, & \text{if $n$ is the product of an even number of distinct primes,}\\
     -1, & \text{if $n$ is the product of an odd number of distinct
       primes,}\\
     0, & \text{otherwise, i.e., if $n$ is not square-free.}
   \end{cases}
 \end{displaymath}
 We now use the approximation
 \eqref{T-approx} for $T(\frac un)$
\begin{equation}
  \label{H-mu}
  R(u)   = \sum_{n=1}^\infty \mu(n) n T(\tfrac un)=
            \sum_{n=1}^\infty \mu(n) \tfrac {u^3}{3n^2} + E_0
%  = \tfrac {u^3}{3\zeta(2)} + E_0        
\end{equation}
 and bound the error
 $E_0$ by
\eqref{bound-E}:
 \begin{align*}
  | E_0| &\le
        \sum_{n=1}^\infty \left|\mu(n) n E(\tfrac un)\right|
  % \\ &
  \le
        \sum_{n=1}^\infty  n E(\tfrac un)
   \\
 &\le
        \sum_{n=1}^{\lfloor u\rfloor} \tfrac {2u^2}{3n}
 +
   \sum_{n=\lfloor u\rfloor+1}^\infty  \tfrac {u^3}{3n^2}
   =\tfrac{2u^2}3 \cdot O(\log u) + \tfrac{u^3}3\cdot O(1/u)%\tfrac1u 
   =O(u^2\log u) 
 \end{align*}
The first term in \eqref{H-mu} can be expressed in terms of the
zeta-function
using the well-known relation \cite[Theorem~287]{HW}
(which also derives from the inclusion-exclusion formula)
\begin{align*}
  % 1\Bigm/
  \sum_{n=1}^\infty \frac {\mu(n)}{n^2}
  &
    =
    % \frac 1{1-\frac1{2^2}}\cdot
    % \frac 1{1-\frac1{2^2}}\cdot
    % \frac 1{1-\frac1{2^2}}\cdot
    % \frac 1{1-\frac1{2^2}}\cdots    
    \biggl(1-\frac1{2^2}\biggr)
    \left(1-\frac1{3^2}\right)
    \left(1-\frac1{5^2}\right) 
    \left(1-\frac1{7^2}\right) \cdots
  \\
  &=
    \frac1{1+\tfrac1{2^2}+\tfrac1{4^2}+\tfrac1{8^2}+\cdots}
   \cdot \frac1{1+\tfrac1{3^2}+\tfrac1{9^2}+\tfrac1{27^2}+\cdots}
   \cdot \frac1{1+\tfrac1{5^2}+\tfrac1{25^2}+\tfrac1{125^2}+\cdots}
    \cdots\\
  &=
    \frac1{\sum_{n=1}^\infty\frac1{n^2}} = \frac1{\zeta(2)} = \frac 6{\pi^2}
.
\end{align*}
We obtain
\begin{displaymath}
%  \label{eq:Ru-final}
    R(u)    = \sum_{n=1}^\infty \mu(n) \tfrac {u^3}{3n^2} + E_0
 = \tfrac {u^3}{3\zeta(2)} + E_0
 = \tfrac {2u^3}{\pi^2} +
 O(u^2\log u)
 .
 \qedhere
\end{displaymath}  
 \end{proof}


==> superpeeling.tex <==
\begin{definition}
\begin{enumerate}
    \item A \emph{superpeeling sequence} is defined just like
    a peeling sequence, except that at any step, additional points may be arbitrarily removed, besides the convex hull vertices.
    \item A \emph{subpeeling sequence} is defined just like
    a peeling sequence, except that at any step, an arbitrary
    subset of the convex hull vertices is removed.
    (VARIATION: after peeling, arbitrary points may be added. (points
    that were just removed, or arbitrary other points.)
\end{enumerate}
\end{definition}

\begin{lemma}
\begin{enumerate}
    \item Let
    $U_0,U_1,U_2,\ldots$
    and
    $U'_0,U'_1,U'_2,\ldots$ be two peeling (or superpeeling) sequences.
(finite or infinite, of the same length?)
(regarded a point sets whose hull is to be taken.)

Then $(U_i\cap U'_i)_{i=0,1,\ldots}$ is a superpeeling sequence.
    \item Let
    $U_0,U_1,U_2,\ldots$
    and
    $U'_0,U'_1,U'_2,\ldots$ be two peeling (or subpeeling) sequences.

Then $(U_i\cup U'_i)_{i=0,1,\ldots}$ is a subpeeling sequence.
\end{enumerate}
\end{lemma}

\begin{proof}
\MS{to be confirmed. (seems obvious) ...}

Obviously, for $A\subseteq B$, a convex hull vertex of $B$ that belongs to $A$ is also a convex hull vertex of $A$. ...
\end{proof}


